Robustness-preserving Lifelong Learning via Dataset Condensation

Lifelong learning (LL) aims to improve a predictive model as the data source evolves continuously. Most work in this learning paradigm has focused on resolving the problem of 'catastrophic forgetting,' which refers to a notorious dilemma between improving model accuracy over new data and retaining accuracy over previous data. Yet, it is also known that machine learning (ML) models can be vulnerable in the sense that tiny, adversarial input perturbations can deceive the models into producing erroneous predictions. This motivates the research objective of this paper - specification of a new LL framework that can salvage model robustness (against adversarial attacks) from catastrophic forgetting. Specifically, we propose a new memory-replay LL strategy that leverages modern bi-level optimization techniques to determine the 'coreset' of the current data (i.e., a small amount of data to be memorized) for ease of preserving adversarial robustness over time. We term the resulting LL framework 'Data-Efficient Robustness-Preserving LL' (DERPLL). The effectiveness of DERPLL is evaluated for class-incremental image classification using ResNet-18 over the CIFAR-10 dataset. Experimental results show that DERPLL outperforms the conventional coreset-guided LL baseline and achieves a substantial improvement in both standard accuracy and robust accuracy.

==> deprecated/experiment.tex <==
\section{Experiments}
\label{sec: experiments}
In this section, we compare our proposed method with two baselines on the robustness-aware CIL task.

% In this section, we first compared the performance in the robustness of two baselines and our method over CIFAR-10 in applying robustness-preserving CIL. Then we also evaluated the performance in the standard CIL to demonstrate the effectiveness of our proposed coreset selection method. Last, we conducted an ablation study to show the relationship between the data ratio and the performance of the three methods. 

\subsection{Experiment setup}
\paragraph*{Datasets \& model architectures.} 
% We evaluated our proposed method on the CIFAR-10 dataset. We split the training dataset into training and validation set with a ratio of $9:1$.  On these datasets, we randomly divide $10$ classes into 5 tasks, each task containing two classes ($10/5 = 2$ classes). The classifier's output dimension will increase by two at each class incremental time.
% And we set the memory bank in the CIL as 100 images per class by default. 
We evaluate the effectiveness of different methods on CIFAR-10 [cite] with ResNet-18 [cite]. The entire dataset with 10 classes in total is randomly divided into 5 tasks, each with 2 classes. The model is trained with a task stream and will adjust the output dimension when a new task arrives. 

\paragraph*{Training details} For each new task, the model will be adversarially trained with both the \textit{complete} new training data and the \textit{selected} old data from the memory bank stored from previous tasks. The coreset selection for the new data will take place after the model training on the current task. We set the size of the memory bank to 100 images per class if not otherwise specified. We leverage the widely adopted 10-step PGD attack [cite] to generate adversarial examples with the attack strength of $8/255$.

\paragraph*{Baselines \& evaluation metrics} We consider two data selection oracles as our baselines:
\textbf{\ding{182} random selection:} randomly samples a subset of the memory bank size from the training set; \textbf{\ding{183} influence score-based selection (IS) \cite{borsos2020coresets}:} select the data with the top influence scores calculated by \eqref{}. For evaluation, we evaluate the performance on \textit{all the tasks} encountered so far. In particular, we look into the \textbf{\ding{172} standard accuracy (SA)}, namely the test accuracy on the clean test set; and \textbf{\ding{173} robust accuracy (RA):}, tested on the perturbed test set. We perform 20-step PGD attack to generate test-time perturbations for evaluation with the same attack strength as training.


% \textbf{(1)} Standard Accuracy (SA) : testing accuracy on the clean test dataset.
% \textbf{(2)} Robust Accuracy (RA): testing accuracy on adversarial examples perturbed from the original test dataset. Here we utilized the $n$-step Projected Gradient Descent (PGD) method to generate the adversarial examples. The perturbation magnitude $\epsilon$ is $8/255$, and the number of steps $n$ is 10 for training and 20 for evaluation by default.

\subsection{Experiment results}

\begin{table}[h]
\begin{center}
\vspace{-1.7em}
\caption{\footnotesize{Performance overview of different methods on the robustness-aware CIL task for the (CIFAR-10, ResNet18) setup. We report the standard accuracy (SA) and robust accuracy (RA) on all the seen tasks and  the average performance (Overall).
% Overall performance of robustness-preserving CIL with different coreset selection methods.
% We reported robust accuracy and standard accuracy on each task ($\mathcal{T}_i$), and overall performance on the whole test dataset (Overall). $\mathcal{T}_1\sim\mathcal{T}_i$ denotes the model has been trained on the $1\to i$ tasks. 
% The robust accuracy is evaluated with $\epsilon = 8/255$. 
The best results are highlighted in \textbf{bold}.}}
\label{tab: robustness}
\begin{threeparttable}
\resizebox{1\linewidth}{!}{
\begin{tabular}{c|c|cc|cc|cc|cc|cc|cc}
\toprule
\multirow{3}{*}{Tasks} & \multirow{3}{*}{Methods} & \multicolumn{10}{c}{CIFAR-10 (SA, RA)} \\ \cmidrule{3-14} 
& & \multicolumn{2}{c|}{$\mathcal{T}_1$ (\%)} & \multicolumn{2}{c|}{$\mathcal{T}_2$ (\%)} & \multicolumn{2}{c|}{$\mathcal{T}_3$ (\%)} & \multicolumn{2}{c|}{$\mathcal{T}_4$ (\%)} & \multicolumn{2}{c|}{$\mathcal{T}_5$ (\%)} & \multicolumn{2}{c}{Overall (\%)}\\ \cmidrule{3-14} 

& & \multicolumn{1}{c|}{SA} & \multicolumn{1}{c|}{RA} & \multicolumn{1}{c|}{SA} & \multicolumn{1}{c|}{RA} & \multicolumn{1}{c|}{SA} & \multicolumn{1}{c|}{RA} & \multicolumn{1}{c|}{SA} & \multicolumn{1}{c|}{RA} & \multicolumn{1}{c|}{SA} & \multicolumn{1}{c|}{RA} & \multicolumn{1}{c|}{SA} & \multicolumn{1}{c}{RA}

\\\midrule
% \multirow{3}{*}{$\mathcal{T}_1$}&Random & 83.65&69.95&- &- &- &-& -& -& -&- & 16.73 &13.99   \\
% &IS &79.20 &70.25&- &- &- &-& -& -& -&-&-&-   \\
% &Ours &83.65 & 69.95 &- &- &- &-& -& -& -&- & 16.73 &13.99  \\
% \midrule
\multirow{3}{*}{$\mathcal{T}_1\sim\mathcal{T}_2$}&Random & 85.65&66.40&71.90 &59.85 &- &-& -& -& -&- & \textbf{31.51} &\textbf{25.25}  \\
&IS&50.40 & 31.80&97.60&77.10 & &- &-& -& -& -&29.60 &21.78      \\
&Ours & 82.90&55.50&73.10 &59.95 &-& -& -& -&- &-& 31.20 &23.09   \\
\midrule
\multirow{3}{*}{$\mathcal{T}_1\sim\mathcal{T}_3$}&Random & 69.10&40.85& 64.50& 21.45&56.85 &41.60& -& -& -&- & {38.09} &20.78   \\
&IS & 46.60&24.90& 63.65 &19.40 &86.20& 58.90& -& -&-&- & \textbf{39.29} &20.64 \\
&Ours&63.70 &49.90&66.40 &21.00 &59.45 &34.90& -& -& -&- & 37.91 &\textbf{21.16}  \\
\midrule
\multirow{3}{*}{$\mathcal{T}_1\sim\mathcal{T}_4$}&Random & 62.30&31.00&66.95 &16.00 &83.45 &65.30& 2.00& 0.15&- & - &42.94 & 22.49\\
&IS& && & & && -& -&- & - &-   \\
&Ours &69.70&45.80 &67.35&28.25& 80.30&54.80 &1.20 & 0.56  & - &- &\textbf{43.71} & \textbf{25.88} \\
\midrule
\multirow{3}{*}{$\mathcal{T}_1\sim\mathcal{T}_5$}&Random & 65.50&39.25&69.00 &16.85 &58.70 &25.40& 56.30& 22.45& 17.95 & 3.95 & 50.69 & 21.58	\\
&IS & && & & && & & -& & - 	\\
&Ours &66.65 &61.90&73.15 &11.85 &61.65 &15.35&44.50&23.95 &23.25 &7.75 &\textbf{53.84}&\textbf{24.16}  	\\
\bottomrule
\end{tabular}}
\end{threeparttable}
\end{center}
\vspace{-5mm}
\end{table}

% \paragraph*{Experiments on the standard CIL} 

\paragraph*{Our method outperforms baselines for robustness preserving.} Tab.\,\ref{tab: robustness} demonstrates the effectiveness of our proposed approach in preserving the robustness. We make some key observations below. \textbf{Firstly}, our method yields an accuracy gap over the baselines on the overall performance at different training stages. As we can see, in each row, the best RA and SA are achieved by our method in most cases. In contrast, the  
\textbf{Secondly}, the accuracy gap between our method  and is enlarged as more tasks join the training.


To further demonstrate the effectiveness of our coreset selection method, we also integrate it with standard CIL.  
Table\,\ref{table:standard} shows the standard accuracy of different methods under the standard CIL framework on the CIFAR-10 dataset. We can observe that our method outperforms other baselines on the average standard accuracy at each stage of CIL. This means that our coreset selection method can also mitigate the issue of forgetting of generalization. 
First, we compared our coreset selection method with two baselines in the robustness-preserving CIL. Table\,\ref{table:robustness} shows the standard accuracy and robust accuracy with class incremental during training. As we can observe, our coreset selection method can improve both standard accuracy and robust accuracy in the robustness-preserving CIL compared to baselines. The results demonstrate that our coreset selection method can mitigate the forgetting of robustness issue further.    


\paragraph*{Abalation study}
We conducted one ablation study to explore the relationship between robustness and  the data ratio which can be saved from old task data during training. Results are shown in the Figure\,\ref{fig:rob_ratio}. 
% \begin{tabular}{c c}
%    \includegraphics[]{Figures/sa_mnist.png}  & \includegraphics[]{Figures/sa_mnist.png} \\
% \end{tabular}
\begin{figure}[h]
    \centering
    \resizebox{0.45\textwidth}{!}{
    \includegraphics[width=\linewidth]{Figures/static_cifar10_std_training (1).pdf}
    \includegraphics[width=\linewidth]{Figures/static_cifar10_ra_training (2).pdf}
    }
\caption{\small{Standard accuracy and Robust accuracy on Cifar10 in static learning, \textbf{(L)} is the clean accuracy over Cifar10. \textbf{(R)} is the robust accuracy over Cifar10 where $\epsilon = 8/255$ }} 
  \label{fig:rob_ratio}
%
\end{figure}
